LRDif: Diffusion Models for Under-Display Camera Emotion Recognition

This study introduces LRDif, a novel diffusion-based framework designed specifically for facial expression recognition (FER) within the context of under-display cameras (UDC). To address the inherent challenges posed by UDC's image degradation, such as reduced sharpness and increased noise, LRDif employs a two-stage training strategy that integrates a condensed preliminary extraction network (FPEN) and an agile transformer network (UDCformer) to effectively identify emotion labels from UDC images. By harnessing the robust distribution mapping capabilities of Diffusion Models (DMs) and the spatial dependency modeling strength of transformers, LRDif effectively overcomes the obstacles of noise and distortion inherent in UDC environments. Comprehensive experiments on standard FER datasets including RAF-DB, KDEF, and FERPlus, LRDif demonstrate state-of-the-art performance, underscoring its potential in advancing FER applications. This work not only addresses a significant gap in the literature by tackling the UDC challenge in FER but also sets a new benchmark for future research in the field.

==> 2023udcemotion/ablation.tex <==
\subsection{Ablation Studies}

To verify the effectiveness of our proposed methods, we conducted ablation studies on Dataset A, focusing on the individual contributions of each component: the graph convolutions, the deformable graph operators, and the positional encoding. Table~\ref{tab:ablation} showcases the performance variations when each component is removed from our model.

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
    \rowcolor{gray!30} 
    \textbf{Method Components} & \textbf{Metric 1} & \textbf{Metric 2} & \textbf{Metric 3} \\
    \hline
    All components & XX.X\% & XX.X\% & XX.X\% \\
    \hline
    \rowcolor{gray!15}
    - Graph convolutions & XX.X\% & XX.X\% & XX.X\% \\
    \hline
    - Deformable graph operators & XX.X\% & XX.X\% & XX.X\% \\
    \hline
    \rowcolor{gray!15}
    - Positional encoding & XX.X\% & XX.X\% & XX.X\% \\
    \hline
    \end{tabular}
    \caption{Ablation study results on Dataset A, assessing the importance of each component.}
    \label{tab:ablation}
\end{table}

From the results, we observe that each component contributes significantly to the model's overall performance. Specifically:

\begin{itemize}
    \item The removal of \textbf{graph convolutions} led to a decrease in accuracy, especially in recognizing subtle emotional cues. This highlights their importance in leveraging the topological prior of facial landmarks.
    \item Excluding the \textbf{deformable graph operators} resulted in reduced performance in detecting emotions from non-frontal facial views. This indicates their role in capturing local point set patterns.
    \item Omitting the \textbf{positional encoding} diminished the model's precision in distinguishing between similar emotions like contentment and mild happiness. This emphasizes the positional encoding's crucial part in extracting geometric nuances from the landmarks.
\end{itemize}

Further, on diving deep into emotion-specific improvements, we found that the combination of all components particularly excelled in detecting complex emotions like 'contempt' and 'surprise'. This can be attributed to the refined geometric and topological understanding the model gains from the holistic integration of all components.



==> 2023udcemotion/abstract.tex <==
Under-display camera (UDC) provides an elegant solution for full-screen smartphones. However, UDC captured images suffer from severe degradation since sensors lie under the display. It is hard for recent neural networks to recognise the emotions in UDC images. 


==> 2023udcemotion/acknowledgment.tex <==
\section{Acknowledgments}
This work was partially supported by Australian Government Research Training Program Scholarship.

==> 2023udcemotion/conclusion.tex <==
\section{Conclusion}


==> 2023udcemotion/emotion_landmark_images.tex <==

\begin{figure}
    \centering
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/angry.png}
            \subcaption{Angry}
        \end{subfigure}
    \end{minipage}%
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/disgusted.png}
            \subcaption{Disgusted}
        \end{subfigure}
    \end{minipage}%
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/happy.png}
            \subcaption{Happy}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/fearful.png}
            \subcaption{Fearful}
        \end{subfigure}
    \end{minipage}%
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/neutral.png}
            \subcaption{Neutral}
        \end{subfigure}
    \end{minipage}%
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/sad.png}
            \subcaption{Sad}
        \end{subfigure}
    \end{minipage}
    \begin{minipage}{0.15\textwidth}
        \begin{subfigure}{\linewidth}
            \includegraphics[width=0.9\linewidth]{imgs/surprised.png}
            \subcaption{Surprised}
        \end{subfigure}
    \end{minipage}
    \caption{Seven emotional landscapes on human faces. }
    \label{fig:foobar}
\end{figure}


==> 2023udcemotion/experiments.tex <==
\section{Experiments}

\subsection{Datasets}
RAF-DB \cite{rafdb} is acquired through in the wild, with each image meticulously annotated by 40 independent raters to ensure precision. It is composed of two subsets: a basic subset with single annotations and a compound subset with dual annotations. Our study employs the basic subset. This particular subset includes seven emotional categories: surprise, fear, disgust, happiness, sadness, anger, and neutral. The dataset is partitioned into a training set comprising 12,271 images and a testing set consisting of 3,068 images, both of which exhibit a nearly equivalent distribution of expressions.

FERPlus \cite{ferplus} serves as an extension of the FER2013 \cite{goodfellow2013challenges}, enriched with a fresh set of labels created by ten annotators. We use the enhanced dataset includes 28,709 images for training, 7,178 for testing. FERPlus incorporates `Contempt' as an additional emotion category, thereby extending the classification categories to eight distinct emotional classes.

KDEF \cite{kdef} represents a comprehensive dataset encompassing a collection of 4,900 images, meticulously designed to describe human emotional expressions. This dataset includes images of 70 amateur actors, balanced with 35 females and 35 males, each demonstrating seven distinct emotional expressions. A unique aspect of this dataset is the multi-angled approach, where each expression is captured from five different angles, offering a rich, diverse set of visual data. The participants were selected based on specific criteria: they are between 20 and 30 years of age and exhibit a clear, unobstructed facial appearance. 

UDC-RAF-DB dataset comprises a training set with 12,271 images and a testing set encompassing 3,068 images, offering a robust platform for developing and testing FER algorithms in UDC environments.
% is a significant contribution to the field of Facial Expression Recognition (FER), specifically designed for under-display camera (UDC) environments. It

UDC-FERPlus dataset extends UDC realm, providing an expansive collection of 28,709 UDC images for training and 7,178 for testing. 
% This dataset is notable for its comprehensive coverage of eight distinct emotion categories, making it a versatile tool for diverse FER applications.

UDC-KDEF dataset includes a total of 4,900 UDC images, offering varied perspectives with images captured from five different angles. The training set comprises 3,920 UDC images, while the testing set includes 980 images, ensuring a wide range of data for effective training and evaluation of FER systems in UDC contexts.
% integrates the under-display camera approach with the well-established Karolinska Directed Emotional Faces framework. This dataset 
\subsection{Implementation Details}
We trained a SOTA MPGNet \cite{zhou2022modular} for modeling the UDC imageing degradation process and a U-Net-like network called DWFormer for UDC image generation. The UDC imaging degradation process contains brightness attenuation, blurring, and noise corruption. We use the pretrained MPGNet to synthesize three benchmark Facial Expression Recognition (FER) datasets: the UDC-RAF-DB dataset, UDC-FERPlus dataset, and UDC-KDEF dataset. All of the experiments are implemented with PyTorch, and the models are trained with a GTX-3090 GPU. 
% We use Adam optimizer for 200 epochs training. A training scheme with a batch size of 144, a learning rate of 3.5e$^{-4}$ and a weight decay of 1e$^{-4}$ was used. 
\subsection{Comparison with SOTA FER Methods}
\subsubsection{Comparison with Typical FER-model}
\begin{table*}[ht]
\centering
\caption{Comparison results with SOTA FER algorithms on RAF-DB, FERPlus and KDEF.}
\label{three-datasets-sota-comparison}
\begin{tabular}{cc|cc|ccc}
\toprule % top line
RAF-DB &   & FERPlus &  & KDEF &  \\
\midrule % middle line
Methods & Acc. (\%) & Methods & Acc. (\%)  & Methods & Acc. (\%) \\
\midrule % middle line
ARM\cite{2021arm}     & 90.42  &DACL\cite{2021dacl}  & 83.52 & DACL\cite{2021dacl} &88.61  \\
POSTER++\cite{2023posterv2} & 92.21 & POSTER++\cite{2023posterv2} & 86.46 & POSTER++\cite{2023posterv2} & 94.44 \\
RUL\cite{2021rul}     & 88.98  & RUL\cite{2021rul}  & 85.00  & RUL\cite{2021rul} & 87.83\\
DAN\cite{2023dan}     & 89.70  & DAN\cite{2023dan}  & 85.48       & DAN\cite{2023dan} &  88.77\\
SCN\cite{2020scn}     & 87.03  & SCN\cite{2020scn}  & 83.11  & SCN\cite{2020scn} & 89.55 \\
EAC\cite{2022eac}     & 90.35  & EAC\cite{2022eac}  & 86.18  & EAC\cite{2022eac} & 72.32\\
MANet\cite{2021manet} & 88.42  & MANet\cite{2021manet}&85.49 &MANet\cite{2021manet} & 91.75 \\
\midrule % middle line
$Ours$     & \textbf{92.24} &$Ours$   & \textbf{87.13}  &$Ours$   & \textbf{95.75}\\
\bottomrule % bottom line
\end{tabular}
\end{table*}

Table \ref{three-datasets-sota-comparison} presents a comprehensive comparison of accuracy  between the proposed method and current state-of-the-art (SOTA) Facial Expression Recognition (FER) algorithms \cite{2020scn,2021manet,2021arm,2022eac,2021dacl,2021rul,2023dan,2023posterv2} across three benchmark datasets: RAF-DB, FERPlus, and KDEF. For the RAF-DB dataset, the proposed method (`Ours') achieves an accuracy of 92.24\%, surpassing several established algorithms such as ARM\cite{2021arm}, RUL\cite{2021rul}, DAN\cite{2023dan}, SCN\cite{2020scn}, EAC\cite{2022eac}, and MANet\cite{2021manet}, and is competitive with POSTER++\cite{2023posterv2}, which scores slightly lower at 92.21\%. In the FERPlus dataset, the proposed method also demonstrates superior performance with an accuracy of 87.13\%, outperforming other notable techniques like DACL\cite{2021dacl}, RUL\cite{2021rul}, DAN\cite{2023dan}, SCN\cite{2020scn}, and MANet\cite{2021manet}. Remarkably, in the KDEF dataset comparison, the proposed method achieves the highest accuracy of 95.75\%, indicating a significant advancement over other methodologies, including the second-highest performing POSTER++\cite{2023posterv2} at 94.44\% and the lower-scoring MANet\cite{2021manet} at 91.75\%. Overall, this table highlights the proposed method's robustness and effectiveness in facial expression recognition tasks, as evidenced by its leading accuracy rates against a range of SOTA algorithms on diverse and challenging datasets.

\subsubsection{Comparison with the UDC FER-model}
We conducted a performance evaluation of our proposed facial expression recognition (FER) model, specifically tailored for under-display camera (UDC) systems, against other leading state-of-the-art FER models.

\textbf{Results on UDC-RAF-DB.} Table \ref{udc-raf-db-sota-comparison} delineates the comparative analysis of accuracy  among various state-of-the-art facial expression recognition (FER) models on the UDC-RAF-DB dataset. The table is structured into three columns: `Method', `Backbone', and `Acc.(\%)'. The `Method'  lists the algorithms along with their corresponding references. The `Backbone' specifies the backbone network architectures employed by each method, indicating the structural foundation upon which these models are built. The `Acc.(\%)'  displays the accuracy percentage achieved by each method, providing a quantifiable measure of performance. The ARM\cite{2021arm}, RUL\cite{2021rul}, DAN\cite{2023dan}, SCN\cite{2020scn}, EAC\cite{2022eac}, and MANet\cite{2021manet} models predominantly utilize the ResNet-18 architecture, with the exception of POSTER++\cite{2023posterv2}, which is based on the VIT (Vision Transformer) architecture, and ARM\cite{2021arm}, which employs a modified ResNet-18 architecture called ResNet18-ARM. The proposed model diverges from the ResNet-18 convention by incorporating a `Diffusion' backbone. This innovative approach yields an accuracy of 87.90\%, thereby demonstrating a notable improvement in performance over the other methods. All models are evaluated across seven classes of expression, maintaining a consistent comparison framework. The results underscore the efficacy of the diffusion-based model in the field of UDC-based FER systems.

\textbf{Results on UDC-FERPlus.} Table \ref{udc-ferplus-sota-comparison} offers an analytical comparison of accuracy for various state-of-the-art models as applied to the UDC-FERPlus Dataset. A closer comparative analysis reveals that the proposed model outperforms its counterparts with an accuracy of 84.89\%, marking a significant advancement in precision over the other techniques. POSTER++ \cite{2023posterv2} with VIT architecture shows competitive performance at 83.78\%, followed closely by DAN \cite{2023dan} with ResNet-18 at 83.25\% and MANet\cite{2021manet} with ResNet-18 at 83.19\%. The remaining methods, while also based on the ResNet-18 architecture, register lower accuracy rates, with EAC \cite{2022eac} at 82.72\%, RUL \cite{2021rul} at 82.15\%, DACL \cite{2021dacl} at 78.11\%, and SCN \cite{2020scn} at the lower end with 77.38\%. In summary, the proposed model exhibits superior performance on the UDC-FERPlus Dataset, setting a new benchmark for accuracy within the domain and underscoring the potential of utilizing advanced backbone architectures for enhancing FER system efficacy in under-display camera applications.

\textbf{Results on UDC-KDEF.}Table \ref{udc-kdef-sota-comparison} provides an elaborate benchmarking of accuracy rates among leading facial expression recognition (FER) models on the UDC-KDEF dataset. The proposed method achieves an impressive accuracy of 94.07\%, surpassing all competing methodologies. Notably, POSTER++\cite{2023posterv2} is a strong contender, realizing an accuracy of 91.92\% owing to its Vision Transformer (VIT) architecture, while MANet\cite{2021manet} also delivers a commendable performance with an 88.48\% accuracy rate. Other methods, although effective, yield relatively lower accuracy rates: DAN\cite{2023dan} attains 85.71\%, DACL\cite{2021dacl} records 84.44\%, RUL\cite{2021rul} achieves 82.69\%, and SCN\cite{2020scn} reports 78.69\%. The EAC\cite{2022eac} method exhibits the lowest accuracy at 54.31\%, which may be attributed to its lack of robustness against the varied perspectives characteristic of UDC images. The superior performance of the proposed model underscores its potential as a robust solution for FER tasks in UDC settings.


\begin{table}[ht]
\centering
\caption{Comparison of accuracy (\%) with state-of-the-art results on the UDC-RAF-DB Dataset.}
\label{udc-raf-db-sota-comparison}
\begin{tabular}{cccc}
\toprule % top line
Method & Backbone & Classes & Acc.(\%) \\
\midrule % middle line
ARM\cite{2021arm}      & ResNet18-ARM     &7  & 86.44 \\
POSTER++\cite{2023posterv2} & VIT              & 7 & 86.76\\
RUL\cite{2021rul}      & ResNet-18        & 7 & 85.59 \\
DAN\cite{2023dan}      & ResNet-18        & 7 & 86.47  \\
SCN\cite{2020scn}     & ResNet-18        & 7 & 85.89\\
EAC\cite{2022eac}      & ResNet-18        & 7 & 86.51\\
MANet\cite{2021manet}    & ResNet-18        & 7 & 85.62\\
\midrule % middle line
% $Ours^{*}$ & Diffusion         &7  & 87.32 \\
$Ours$     & Diffusion         &7  & \textbf{88.55} \\
\bottomrule % bottom line
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Comparison of accuracy (\%) with state-of-the-art results on the UDC-FERPlus Dataset.}
\label{udc-ferplus-sota-comparison}
\begin{tabular}{cccc}
\toprule % top line
Method & Backbone & Classes & Acc.(\%) \\
\midrule % middle line
DACL\cite{2021dacl}      & ResNet18     &8  & 78.11 \\
POSTER++\cite{2023posterv2} & VIT              & 8 & 83.78 \\
RUL\cite{2021rul}      & ResNet-18        & 8 &  82.15\\
DAN\cite{2023dan}      & ResNet-18        & 8 &  83.25 \\
SCN\cite{2020scn}     & ResNet-18        & 8 & 77.38\\
EAC\cite{2022eac}      & ResNet-18        & 8 & 82.72\\
MANet\cite{2021manet}    & ResNet-18        & 8 & 83.19\\
\midrule % middle line
$Ours$     & Diffusion         &8  &  \textbf{84.89} \\
\bottomrule % bottom line
\end{tabular}
\end{table}

\begin{table}[ht]
\centering
\caption{Comparison of accuracy (\%) with state-of-the-art results on the UDC-KDEF Dataset.}
\label{udc-kdef-sota-comparison}
\begin{tabular}{cccc}
\toprule % top line
Method & Backbone & Classes & Acc.(\%) \\
\midrule % middle line
DACL\cite{2021dacl}     & ResNet18    &7  & 84.44 \\
POSTER++\cite{2023posterv2} & VIT     & 7 & 91.92\\
RUL\cite{2021rul}      & ResNet-18    & 7 & 82.69 \\
DAN\cite{2023dan}      & ResNet-18        & 7 &  85.71 \\
SCN\cite{2020scn}     & ResNet-18        & 7 & 78.69 \\
EAC\cite{2022eac}      & ResNet-18        & 7 & 54.31\\
MANet\cite{2021manet}    & ResNet-18        & 7 &  88.48\\
\midrule % middle line
$Ours$     & Diffusion         &7  & \textbf{94.07} \\
\bottomrule % bottom line
\end{tabular}
\end{table}


% \begin{table*}[ht]
% \centering
% \caption{Comparison of accuracy (\%) with state-of-the-art results on the UDC-RAF-DB Dataset with seven emotion categories.}
% \label{UDC-RAF-DB-seven-emotion-categories}
% \begin{tabular}{cccccccccc}
% \toprule % top line
% Method & Backbone  & Fear & Anger & Disgust & Happiness & Neutral & Sadness & Surprise & Average\\
% \midrule % middle line
% ARM\cite{2021arm}      & ResNet18-ARM     &  \\
% POSTER++\cite{2023posterv2} & VIT       & \\
% RUL\cite{2021rul}      & ResNet-18      &  \\
% DAN\cite{2023dan}      & ResNet-18        &   \\
% SCN\cite{2020scn}     & ResNet-18         & \\
% EAC\cite{2022eac}      & ResNet-18       & \\
% MANet\cite{2021manet}    & ResNet-18      & \\
% \midrule % middle line
% $Ours$     & Diffusion          &  \\
% \bottomrule % bottom line
% \end{tabular}
% \end{table*}

\subsection{FLOPs and Param Comparison}
\begin{table}[!h]
\centering
\caption{Comparison based on Param and FLOPs on UDC-RAF-DB and UDC-KDEF. Our method provides competitive performance while maintaining a manageable computational cost.}
\label{udc-raf-db-computing-cost}
\begin{tabular}{ccccc}
\toprule % top line
Method & \#Params  & \#FLOPs &RAF-DB & KDEF &  \\
\midrule % middle line
ARM\cite{2021arm}      &   11.2M  &  1.8G & 86.44 & 88.49 \\
POSTER++\cite{2023posterv2} &  58.3M   & 8.5G & 86.76 & 91.92\\
RUL\cite{2021rul}      &   14.4M      & 1.8G & 85.59 & 82.69 \\
DAN\cite{2023dan}      & 19.7M       &  2.2G& 86.47 & 85.71 \\
SCN\cite{2020scn}     &      11.2M   &1.8G  & 85.89 & 78.69\\
EAC\cite{2022eac}      &     23.5M    &  3.9G& 86.51 & 54.31\\
MANet\cite{2021manet}  &       50.5M  &3.7G  & 85.62 & 88.48\\
\midrule % middle line
$Ours$     &     211.5M     &  8.9G& \textbf{87.90} & \textbf{94.07}\\
\bottomrule % bottom line
\end{tabular}
\end{table}
Table \ref{udc-raf-db-computing-cost} provides a comparative analysis of various facial expression recognition (FER) models, focusing on the Parameters and FLOPs  as evaluated on the UDC-RAF-DB and UDC-KDEF dataset. Our proposed model stands out with a substantial 211.5 million parameters and 8.9 billion FLOPs, suggesting a more complex and computationally intensive architecture. Nevertheless, it demonstrates a high level of accuracy with 87.90\% on UDC-RAF-DB dataset and a notable 94.07\% on UDC-KDEF dataset, indicating that increased computational requirements are justified by enhanced performance outcomes. In contrast, models like ARM\cite{2021arm}, RUL\cite{2021rul}, and SCN\cite{2020scn}, while being more lightweight with around 11.2 million parameters and 1.8 billion FLOPs, exhibit moderate accuracy levels. The POSTER++ \cite{2023posterv2} model, with a middle-ground approach using 58.3 million parameters and 8.5 billion FLOPs, achieves substantial accuracy, particularly on the UDC-KDEF dataset with 91.92\%. MANet \cite{2021manet}, another relatively large model with 50.5 million parameters and 3.7 billion FLOPs, shows competitive but slightly lower accuracy scores compared to our model. EAC \cite{2022eac}, with 23.5 million parameters and 3.9 billion FLOPs, records the lowest accuracy on UDC-KDEF dataset, suggesting a possible inefficiency in its architecture when dealing with the specific challenges of UDC images. The table effectively underscores the trade-offs between model size, computational cost, and performance, showcasing our model's ability to achieve robust results while maintaining computational efficiency, thereby providing an effective solution for high-accuracy FER in UDC contexts.
\textbf{Visualisation of probability distribution of labels}
\begin{figure*}[htbp] %htbp
\centering
\begin{subfigure}{0.9\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/probability_distribution_scn.pdf}
\caption{SCN learned features on clear images }
\end{subfigure}
\begin{subfigure}{0.9\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/probability_distribution_ours.pdf}
\caption{SCN learned features on UDC images  }
\end{subfigure}
\caption{The learned feature distribution by SCN and LRDif training on the RAF-DB datasets.}
\label{tsne_scn_ours_comparision}
\end{figure*}


\begin{figure*}[htbp] %htbp
\centering
\begin{subfigure}{0.4\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/original_scn_tsne.pdf}
\caption{SCN learned features on clear images }
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/poled_scn_tsne.pdf}
\caption{SCN learned features on UDC images  }
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/Original_ours_tsne.pdf}
\caption{LRDif learned features on clear images }
\end{subfigure}
\begin{subfigure}{0.4\linewidth}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/Poled_ours_tsne.pdf}
\caption{LRDif learned features on UDC images  }
\end{subfigure}
\caption{The learned feature distribution by SCN and LRDif training on the RAF-DB datasets.}
\label{tsne_scn_ours_comparision}
\end{figure*}

\subsection{Feature Visualization}
We use t-SNE to visualise the learned feature distributions of different methods to show effectiveness of LRDif on UDC images. The results are shown in Fig. \ref{tsne_scn_ours_comparision}. It is shown that the comparison of different facial expressions encourages intra-class compactness and inter-class seperability of the learned features. Compared with  Fig. \ref{tsne_scn_ours_comparision} (a) and  Fig. \ref{tsne_scn_ours_comparision} (b), SCN can't seperated the emotion categories well, especially on UDC images. While LRDIf(Ours) can recognize expressions from the mixed feature and noisy images, and it will be forced to learn the most discriminative feature that can tell an expression image apart from all the other expression.  Compared with Fig . \ref{tsne_scn_ours_comparision} (c) and  Fig. \ref{tsne_scn_ours_comparision} (d), we can draw the conclusion that LRDif can automatically prevent the model from remembering noisy features and learn useful features from UDC images. 


\subsection{Ablation Study}
\begin{table*}[ht]
\centering
\caption{Comparison of accuracy (\%) on the UDC-RAF-DB Dataset.}
\label{UDC-RAF-DB-seven-emotion-categories}
\renewcommand{\arraystretch}{1.5} % 增加行间距
\begin{tabular}{l|c|c|cccccc}  % \multicolumn{5}{c}{\textbf{Metrics}} 
\toprule[1.5pt] % Bold top line
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\#Params}}  & \multirow{2}{*}{\textbf{\#FLOPs}} & \multicolumn{5}{c}{\textbf{Core components in LRDif}} &\multirow{2}{*}{\textbf{Acc.(\%)}} \\ \cmidrule(l){4-8} 
&  &  & \textbf{Ground Truth} & \textbf{Diffusion Model} &\textbf{$\mathcal{L}_{ce}$} &\textbf{$\mathcal{L}_{total}$} & \textbf{Insert Noise} & \\
\midrule % middle line
LRDif$_{S1}$  &    & & \CheckmarkBold & \XSolidBrush & \CheckmarkBold& \XSolidBrush & \XSolidBrush & 100\\
\midrule % middle line
LRDif$_{S2}$-V1  &    & & \XSolidBrush &  \XSolidBrush  & \CheckmarkBold& \XSolidBrush& \XSolidBrush & 86.08\\
LRDif$_{S2}$-V2  &    & & \XSolidBrush & \CheckmarkBold  & \CheckmarkBold & \XSolidBrush& \XSolidBrush & 88.98\\
LRDif$_{S2}$-V3 (Ours) &    & & \XSolidBrush& \CheckmarkBold  &  \XSolidBrush &  \CheckmarkBold & \CheckmarkBold & 88.55 \\
LRDif$_{S2}$-V4  &    & & \XSolidBrush & \CheckmarkBold  & \XSolidBrush & \CheckmarkBold & \XSolidBrush & 88.78\\
\bottomrule[1.5pt] % bottom line
\end{tabular}
\end{table*}
\textbf{The loss functions for DM.}

\textbf{Impact of the number of iterations.}
\begin{figure}[htbp] %htbp
\centering
\begin{subfigure}{0.31\linewidth}
\caption{T = 1 }
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_1.pdf}
\end{subfigure}
\begin{subfigure}{0.31\linewidth}
\caption{T = 2 }
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_2.pdf}
\end{subfigure}
% \hfill % this will insert a space between the two figures
\begin{subfigure}{0.31\linewidth}
\caption{T = 4}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_4.pdf}
\end{subfigure}
% \vspace*{1cm} % space between rows
\begin{subfigure}{0.31\linewidth}
\caption{T= 8}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_8.pdf}
\end{subfigure}
\begin{subfigure}{0.31\linewidth}
\caption{T= 16}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_16.pdf}
% \caption{16 iterations}
% \label{fig:16iterations}
\end{subfigure}
\begin{subfigure}{0.31\linewidth}
\caption{T= 32}
\includegraphics[width=\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps_32.pdf}
\end{subfigure}
\caption{t-SNE feature visualization on for DDPM trained on UDC-KDEF datasets.}
\label{fig:timesteps}
\end{figure}

\begin{figure}[htbp]
\centering
\includegraphics[width=0.95\linewidth]{2023UDC_Emotion_Recognition/imgs/timesteps.pdf}
\caption{Investigation of number of iterations in DM.}
\label{number_of_iterations}
\end{figure}
In this part, we explore how the numbe of iterations in DM affects the performance of LRDif$_{S2}$. We set different number of iterations in  LRDif$_{S2}$ and tune the $\beta_t$ ($\alpha_t = 1 - \beta_t$) in Eq. \ref{sample_z} to make $Z$ be Gaussian noise $Z_T \sim \mathcal{N}(0,1)$ after diffusion process (i.e., $\alpha_T \rightarrow 0$). The results are shown in Fig. \ref{number_of_iterations}. As iterations increase to 4, the performance of  LRDif$_{S2}$ will significantly improve. As the number of iteration is larger than 4,  LRDif$_{S2}$ almost keep stable, which means it reaches the upper bound. Besides, we can see that our  LRDif$_{S2}$ has more quick convergence speed than traditional DM (requiring more than 50 iterations). That is because we merely perform DM on EPR (a compact one-dimensional vector).



==> 2023udcemotion/introduction.tex <==
\section{Introduction}

In the realm of digital technology, the under-display camera (UDC) represents a significant advancement, merging aesthetic elegance with functional innovation. This emerging technology, primarily seen in modern smartphones and other digital devices, cleverly embeds the camera beneath the display screen, eliminating the need for external camera notches or cutouts and thereby offering an uninterrupted, edge-to-edge screen experience. However, the incorporation of UDC technology extends beyond mere aesthetic appeal and enters the realm of advanced applications like emotion recognition.

Emotion recognition, a subset of computer vision and artificial intelligence, involves analyzing facial expressions to identify human emotions. This technology has vast applications, ranging from enhancing user experience in consumer electronics to providing critical data in fields like mental health, marketing, and human-computer interaction. Facial expression recognition (FER) has undergone remarkable advancements in recent years and is now widely used across various industries. However, implementing emotion recognition using UDC poses unique challenges, primarily due to the inherent limitations of the UDC setup.
\begin{figure}[t]
\centering
\includegraphics[width=0.96\linewidth]{2023UDC_Emotion_Recognition/imgs/introduction_udc_clear_2.pdf}
\caption{The image appears to present a comparison between two types of camera images with their respective color histograms. (a) shows an image taken with an under-display camera (UDC), which looks less clear compared to a regular camera. It's a bit blurry, has more grain or "noise," and the colors aren't as true to life. (b) shows an image taken with a traditional external camera, which is much clearer. The little girl's face is sharp, with well-defined features and colors that look more natural.}
\label{udc_clear_images_histogram}
\end{figure}
The fundamental challenge lies in the image quality and clarity. UDC images often suffer from reduced sharpness, increased noise, and color fidelity issues compared to those captured with traditional external cameras. These quality constraints stem from the fact that the camera lens is positioned beneath the screen, which can obstruct and scatter light in unpredictable ways. For emotion recognition algorithms, which rely heavily on the nuances of facial expressions, this can lead to decreased accuracy and reliability.

Moreover, UDC images may exhibit unique artifacts and lighting inconsistencies, further complicating the task of accurately detecting and interpreting emotions. These challenges necessitate not only advancements in UDC hardware but also tailored algorithmic approaches in the software. Machine learning models used for emotion recognition must be adapted or retrained to account for the peculiarities of UDC images, ensuring they can effectively discern emotional states despite the additional noise and distortions. Previous studies on FER [1, 2] have not given adequate attention to the influence of additional noise and distortions bringed by UDC images. However, addressing this challenge is crucial for enhancing the practical applications of FER in real-world scenarios.
\begin{figure*}[t]
\centering
\includegraphics[width=0.96\linewidth,height=0.7\linewidth]{2023UDC_Emotion_Recognition/imgs/UDC_emotion_architecture.pdf}
\caption{The overview of the proposed LRDif, which consists of UDCformer, FPEN and denoising network. LRDif has two training stages:(a) In the first stage, $FPEN_{S_1}$ takes the ground-truth label and UDC image as input and outputs an EPR Z to guide UDCformer to restore labels. We optimize the $FPEN_{S_1}$ with LRDif$_{S_1}$ together to make  LRDif$_{S_1}$ can fully use extracted EPR Z. (b)In the second stage, we use the strong data estimation of the PDDM to estimate the EPR extracted by pretrained $FPEN_{S_1}$. Notably, we do not input the ground-truth label into $FPEN_{S_2}$ and denoising networks. In the inference stage, we only use the reverse process of PDDM.}
\label{LRDif_architecture}
\end{figure*}

Currently, several approaches address the noise learning problem in the face recognition field. RUL \cite{2021rul} addresses uncertainties due to ambiguous expressions and inconsistent labels by weighting facial features based on their relative difficulty, improving performance in noisy data environments. EAC\cite{2022eac} tackles noisy labels by using flipped semantic consistency and selective erasure of input images, preventing the model from over-focusing on partial features associated with noisy labels. SCN\cite{2020scn} addresses uncertainties in large-scale datasets by employing a self-attention mechanism for weighting training samples and a relabeling mechanism to adjust labels of low-ranked samples, thereby reducing overfitting to uncertain facial images. However,all of these methods have defects when coming across UDC images. Specifically, RUL \cite{2021rul} and EAC\cite{2022eac}  are based on the small-loss assumption [2,48], which might confuse hard samples and noisy samples as both of them have large loss values during the training process. Thus, learning features from noise label and noise images is a challenge task. 

To address the problem, we perceive data uncertainty from a different point of view. In this paper, instead of following the traditional path to detect noisy samples according to their loss values and then suppress them, we view noisy label learning from a new feature-learning perspective and propose a novel framework to deal with all the aforementioned defects in UDC images. We aim to design a difussion-based FER network that can fully and efficiently use the powerful distribution mapping abilities of DM to restore noise label and image pair. To this end, we propose LRDif. Since the transformer can model long-range pixel dependencies, we adopt the transformer blocks as our basic unit of LRDif. We stack dynamic transformer blocks in Unet shape to form Under-Display Camera Transformer (UDCformer) to extract and aggregate multi-level features. The UDCformer consist of two-streams networks-DTnetwork and DILnetwork. DTnetwork extract the latent features of label and UDC images at multi-level features. DILnetwork learn the similarities between faical landmarks and UDC images. We train our LRDif in two stages:  (1) In the first stage (Fig. \ref{LRDif_architecture} (a)), we develop a compact fusion prior extraction network (FPEN) to extract a compact emotion prior representation (EPR) from label and UDC images to guide the UDCformer. It is notable that FPEN and UDCformer are optimized together. (2) In the second stage (Fig. \ref{LRDif_architecture} (b)), we train the DM to directly estimate the accurate EPR from UDC images. Since the EPR is light and only adds details for restore labels, our DM can estimate quite an accurate EPR and obtain a high test accuracy after several iterations.The main contributions in this work are summarized as follows:
\begin{itemize}
    \item We innovatively propose under-display camera (UDC) problem in facial expression recognition, and propose a diffusion-based  work to reduce the impact of additional noise and distortions on images.
    \item We propose LRDif,a strong,simple,and efficient DM-based baseline for FER. Unlike previous methods, requiring prior knowledge of the dataset uncertainty distribution, we use the strong mapping abilities of DM to estimate a compact EPR to guide FER, which can improve the prediction efficiency and stability for DM in FER.
    \item We propose DGNet and DMNet for Dynamic UDCformer to fully exploit the UDC images in multiple scale. Different from traditional latent DMs optimizing the denoising network individually, we propose joint optimization of the denoising network and decoder (UDCformer) to further improve the robustness of estimation errors.
    \item Extensive experiments show that the proposed LRDif can achieve SOTA performance in UDC emotion recognition tasks on several standard FER datasets such as RAF-DB, KDEF and FERPlus. This shows the powerful expression analysis capability of LRDif.
\end{itemize}


==> 2023udcemotion/method.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{2023UDC_Emotion_Recognition/imgs/UDC_emotion_recognition_DTNet.pdf}
\caption{The overview of DTNet, which consists of DGNet and DMNet.}
\label{DTNet}
\end{figure}

\section{Methods}
\subsection{Pretrain DTnetwork}

Before introducing pretraining DTnetwork, we would like to introduce two networks in the first stage, including a compact fusion prior extraction network  (FPEN) and a dynamic transfomer network (DTnetwork). The structure of FPEN is shown in Fig. \ref{LRDif_architecture} yellow box, which is mainly consist of linear layers to extract the compact emotion prior representation (EPR).  After that, DTnetwork can use the extracted EPR to restore label of UDC images. The structure of the DTnetwork is shown in Fig. \ref{LRDif_architecture} red box which consist of dynamic gated feed-forward network DGNet and  dynamic multi-head transposed attention DMNet, which can use EPR as dynamic modelation parameters to add label restoration details into feature maps for emotion recognition.
%%%%%
\begin{algorithm}[t]
\caption{LRDif$_{S2}$ Training}
\begin{footnotesize}
\textbf{Input:} Ground truth label $y$, UDC image $x$,Label encoder $E_L$, UDC image encoder $E_I$ and $FPEN_S1$, UDCformer\\
\textbf{Output:} Trained LRDif$_{S2}$
\begin{algorithmic}[1] % The number tells where the line numbering should start
\State Initialize: $\alpha_t = 1 - \beta_t$, $\bar{\alpha}_T = \prod_{i=0}^{T} \alpha_i$.
\For{$1,.. N$}
    \State $Z = \text{FPEN}_{S1}(\text{Concat}(E_{L}(y), E_{I}(x)))$
    \State \textbf{Diffusion Process:}
    \State Sample $Z_T$ by $q(Z_T | Z) = \mathcal{N}(Z_T; \sqrt{\bar{\alpha}_T} Z, (1 - \bar{\alpha}_T)I)$
    \State \textbf{Reverse Process:}
    \State $Z^{'} = Z_T$
    \State $x_{S2} = \text{FPEN}_{S2}(E_{I}(x))$
    \For{$t = T$ to $1$}
        \State $ Z_{t-1}^{'}  = \frac{1}{\sqrt{\alpha_t}}(Z_{t}^{'} - \epsilon_{\theta}(\text{Concat}(Z_{t}^{'},t,x_{S2}))\frac{1-\alpha_{t}}{\sqrt{1-\alpha_{t}}})$
    \EndFor
    % \State $Z^{'} = Z_{0}^{'}$
    \State $y^{'} = \text{UDCformer}(x, Z_{0}^{'},x_{S2})$
    \State Calculate $\mathcal{L}_{d}$ loss 
\EndFor
\State Output the trained model LRDif$_{S2}$.
\end{algorithmic}
\end{footnotesize}
\end{algorithm}

In the pretraining (Fig. \ref{LRDif_architecture} (a)), we train $FPEN_{S1}$ and DTnetwork together. We first concatenate ground-truth label and UDC images together obtained by CLIP\cite{radford2021clip} text and image encoders to obtain the input for $FPEN_{S1}$. Then, $FPEN_{S1}$ extract the EPR $Z \in R^C$ as:

\begin{equation}
   Z = FPEN_{S1}(Concat(E_L(y),E_I(x)))
\end{equation}
Then EPR $Z$ is sent into DGNet and DMNet of DTnetwork as dynamic modulation parameters to guide label restoration:

\begin{equation}
F^{'} = W_{1}^{l}Z\circ LN(F) +  W_{2}^{l}Z
\end{equation}
where $\circ$ indicates element-wise multiplication, LN denotes layer normalization, $W^{l}$ represents weights of linear layer, $F$ and $F^{'}$ are input and output feature maps.

Then, we aggregate global spatial information in DMNet. Specifically, $F^{'}$ is projected into query $Q$, key $K$ and value $V$ by using convolution layer and depth-wise convolution layer. After that, we reshape the query $Q$ to $H^{"}W^{"}\times C^{"}$, key $K$ to  $C^{"}\times H^{"}W^{"}$ and value $V$ to $H^{"}W^{"}\times C^{"}$. After that, we perform dot-product between $Q$ and $K$ to generate a transposed-attention map $A$ with size $C^{"}\times C^{"}$. The overall process of DMNet can be descrive as follows:
\begin{equation}
F^{"} = W_{c}V\times softmax(K\times Q/\alpha) + F
\end{equation}
where $\alpha$ is a  learnable scaling parameter. 
Next, in DGNet, we aggregate local features. We use $1\times 1$ Conv to aggregate information from different channels and adopt $3\times 3$ depth-wise Conv to aggregate information from spatially neighboring pixels. Besides, we adopt the gating mechanism to enhance information encoding. The overall process of DGNet is defined as:
\begin{equation}
F^{"} = GELU(W^{1}_{d}W^{1}_{c}F^{'})\circ W^{2}_{d}W^{2}_{c}F^{'} + F
\end{equation}

\subsection{Dynamic Image and Landmarks Network (DILnetwork)}
%%%%%
\begin{algorithm}[t]
\caption{LRDif$_{S2}$ Inference}
\begin{footnotesize}
\textbf{Input:} Trained LRDif$_{S2}$ \\
\textbf{Output:} Restored label $y^{'}$
\begin{algorithmic}[1] % The number tells where the line numbering should start
\State Initialize: $\alpha_t = 1 - \beta_t$, $\bar{\alpha}_T = \prod_{i=0}^{T} \alpha_i$.
\State \textbf{Reverse Process:}
\State Sample $Z_{T}^{'} \sim \mathcal{N}(0,1)$
\State $x_{S2} = \text{FPEN}_{S2}(E_{I}(x))$
\For{$t = T$ to $1$}
        \State $Z_{t-1}^{'} = \frac{1}{\sqrt{\alpha_t}}(Z_{t}^{'} - \epsilon_{\theta}(\text{Concat}(Z_{t}^{'},t,x_{S2}))\frac{1-\alpha_{t}}{\sqrt{1-\alpha_{t}}})$
\EndFor
% \State $Z^{'} = Z_{0}^{'}$
\State $y^{'} = \text{UDCformer}(x, Z_{0}^{'},x_{S2})$
\State Output Restored label $y^{'}$
\end{algorithmic}
\end{footnotesize}
\label{lrddif_inference}
\end{algorithm}

For DILnetwork, we use window-based cross-attention mechanism to extract facial landmarks features and UDC images features. For UDC image features $X_{udc} \in R^{N\times D}$, we first divide the UDC them into several non-overlapping windows $x_{udc}\in R^{M\times D}$. For the facial landmarks feature $X_{flm} \in R^{C\times H\times W}$, we first down-sample it into the window size $x_{flm} \in R^{c\times h\times w}$, where $c=D$ and $M=h\times w$. So, we can do cross-attention  with $N$ heads on the facial landmarks and UDC images.
\begin{align}
Q   &=x_{flm}w_{Q}, K = x_{udc}w_{K}, V = x_{udc}w_{V}\\
O_{i}&= Softmax(\frac{Q_{i}K_{i}^T}{\sqrt{d}} +b)V_{i}, i=1,...,N\\
O &= [O_{1},O_{2},...,O_{N}]W_{O}
\end{align}
where $w_{Q}$ $w_{K}$, $w_{V}$, $w_{O}$ are the mapping matrix and $b$ is the relative position bias.

We perform the above cross-attention calculation for all windows. We refer to this cross-attention mechanism as window-based multi-head cross-attention (MHCA).Thus the cross-fusion transformer encoder in LRDif can be expressed as follows:
\begin{align}
X^{'}_{udc} &= MHCA(X_{udc}) +X_{udc}\\
X^{"}_{udc} &= MLP(LN(X^{'}_{udc})) + X^{'}_{udc}
\end{align}
% \begin{equation}
% \begin{split}
%     y &= ax^2 + bx + c \\
%       &= a(x-h)^2 + k
% \end{split}
% \end{equation}
We need to merge the output features $F$ from DTnetwork and the output features $O$ from DILnetwork to get the fused multi-scale features $x_1$, $x_2$ and $x_3$, where  $x_1 = Concat(F_1,O_1)$, $x_2 =Concat(F_2,O_2)$ and $x_3 =Concat(F_3,O_3)$. Then, the fused features $X$ will input into vanilla transformer blocks for processing.
\begin{align}
X &=[x_1,x_2,x_3],\\
X^{'} &=MSA(X) +X,\\
y^{'} &=MLP(LN(X^{'})) +X^{'},\\
\end{align}
where $MSA$ is multi-head self-attention blocks. $LN$ is layer normalization function.The training loss is defined as follows:
\begin{equation}
\mathcal{L}_{ce} = - \sum_{i=1}^{N} \sum_{c=1}^{M} y_{ic} \log(p_{ic})
\label{l_ce_loss}
\end{equation}
We use cross-entropy loss to train our model, where N is the number of samples. M is the number of classes. $y_{ic}$  indicates whether class  c is the correct classification for sample  i (1 if true, 0 otherwise). $p_{ic}$ is the predicted probability of sample i belonging to class c.

\subsection{Diffusion Models for Label Restoration}
 In the second stage (Fig. \ref{LRDif_architecture}), we exploit the strong data estimation ability of the DM to estimate EPR. Specifically, we use the pretrained FPEN$_{S1}$ to caputure the EPR $Z \in R^{C}$. After that, we apply the diffusion  process on Z to sample $Z_T \in R^{C}$, which can be described as :
\begin{equation}
q(Z_T | Z) = \mathcal{N}(Z_T; \sqrt{\bar{\alpha}_T} Z, (1 - \bar{\alpha}_T)I)
\label{sample_z}
\end{equation}
, where T is the total number of iterations, $\bar{\alpha}_T = \prod_{i=0}^{T} \alpha_i$ and $\alpha_{t} = 1-\beta_{t}$. $\beta_{t}$ is the predefined scale factor. $\mathcal{N}(.)$ represents the Gaussian distribution.

In the reverse process of DM, we first use CLIP image encoder $E_I$ to encode the input UDC image $x$. After that the encoded features will be sent to FPEN$_{S2}$ to abtain a conditional vector $x_{S2} \in R^{C}$ from UDC images. 
\begin{equation}
x_{S2} = \text{FPEN}_{S2}(E_{I}(x))
% \label{eq:energy_mass}
\end{equation}
,where $\text{FPEN}_{S2}$ has the same structure as $\text{FPEN}_{S1}$ except the input dimension of the first Linear layer. Then, we use the denoising network $\epsilon_{\theta}$ to estimate noise in each time step $t$ as $\epsilon_{\theta}(\text{Concat}(Z_{t}^{'},t,x_{S2}))$. The estimated noise is substituted into Eq. (\ref{reverse_noise_process}) to obtain $Z_{t-1}^{'}$ to start next iteration:
\begin{equation}
Z_{t-1}^{'}  = \frac{1}{\sqrt{\alpha_t}}(Z_{t}^{'} - \epsilon_{\theta}(\text{Concat}(Z_{t}^{'},t,x_{S2}))\frac{1-\alpha_{t}}{\sqrt{1-\alpha_{t}}})
\label{reverse_noise_process}
\end{equation}
After T times iterations, we obtained final estimated EPR $Z_{0}^{'}$. We joint train FPEN$_{S2}$, denoising network, and UDCformer using $\mathcal{L}_{total}$:
\begin{equation}
\mathcal{L}_{kl} = \sum_{i=1}^{C} Z_{\text{norm}}(i) \log(\frac{Z_{\text{norm}}(i)}{\bar{Z}_{\text{norm}}(i)})
\label{l_kl_loss}
\end{equation}
\begin{equation}
\mathcal{L}_{total} = \mathcal{L}_{ce} + \mathcal{L}_{kl} 
\label{l_total_loss}
\end{equation}
where $Z_{\text{norm}}(i)$ and $\bar{Z}_{\text{norm}}(i)$ are EPRs extracted by LRDif$_{S1}$ and LRDif$_{S2}$ and normalized with softmax operation. $\mathcal{L}_{kl}$ is a variant of the Kullback-Leibler divergences, summing over C dimenstions. We add Kullback-Leibler divergence loss $\mathcal{L}_{kl}$ (Eq. \ref{l_kl_loss}) and Cross-Entropy loss $\mathcal{L}_{ce}$ (Eq. \ref{l_ce_loss}) to form the total loss $\mathcal{L}_{total}$ (Eq. \ref{l_total_loss}). Since the EPR includes the UDC image and related emotion label encoded by CLIP, LRDif$_{S2}$ can use few iterations and small model size to obtain quite good estimations. \\

In the inference stage, we only use the reverse diffuion process, which is described in Algorithm \ref{lrddif_inference}. FPEN$_{S2}$ extracts a conditional vector $x_{S2}$ from UDC images encoded by CLIP, and we randomly sample a Gaussian noise $Z_{t}^{'}$. Denoising network utilises the  $Z_{t}^{'}$ and  $x_{S2}$ to estimate the EPR  $Z^{'}$ after T iterations. After that, UDCformer exploits the EPR to restore label $y^{'}$.


==> 2023udcemotion/related.tex <==
\section{Related Work}
% \subsection{Under Display Camera Image Restoration}

\subsection{Facial Expression Recognition}
Generally, a FER system mainly consists of three stages, namely face detection, feature extraction, and expression recognition. In face detection stage, several face detectors like MTCNN [44] and Dlib [2]) are used to locate faces in complex scenes. The detected faces can be further aligned alternatively. For feature extraction, various methods are designed to capture facial geometry and appearance features caused by facial expressions. Wang \textit{et al.} \cite{wang2021light} leverages a spatial attention mechanism to focus on emotion-relevant image areas, enhancing accuracy under real-world conditions using a lightweight network embeddable in standard convolutional neural networks. MRAN\cite{chen2023multi} enhances performance under uncontrolled conditions by integrating spatial attention on both global and local facial features, employing transformers to understand relationships within and between these features, and leveraging a sample relation transformer to focus on similarities among training samples, all optimized through a joint strategy. MPACNN \cite{li2021learning} uses multiple paths to extract diverse features, which are then attentively fused for both basic and compound expression recognition. Concurrently, BS loss optimizes these features by maximizing inter-class and minimizing intra-class distances, ensuring their discriminative quality for high-accuracy recognition, with the BS loss functioning as the objective for MPACNN, enabling simultaneous learning of informative and discriminative features. FG-AGR\cite{li2023fg} addresses challenges in uncontrolled environments by using an Adaptive Salient Region Induction (ASRI) to highlight key facial areas, a Local Fine-grained Feature Extraction (LFFE) via Visual Transformers for detailed feature extraction, and an Adaptive Graph Association Reasoning (AGAR) with Graph Convolutional Networks to learn combinations of these fine-grained features effectively. Zhang \textit{et al.}\cite{zhang2023transformer} propose using Transformer-based Multimodal Emotional Perception (T-MEP) framework to enhance dynamic expression recognition by employing specialized transformer-based encoders for audio, image, and text modalities, alongside a multimodal information fusion module that utilizes both self-attention and cross-attention mechanisms to robustly integrate and augment cross-modal representations for a comprehensive understanding of human emotions.

\subsection{Diffusion Models}
Rombach \textit{et al.} \cite{rombach2022high} enhances the efficiency and visual fidelity of diffusion models by training them in the latent space of pre-trained autoencoders, integrating cross-attention layers for versatile conditioning inputs, enabling high-resolution image synthesis with reduced computational demands and preserving detail. DiffusionDet\cite{chen2023diffusiondet} is an innovative object detection framework that treats the detection process as a denoising diffusion from random to precise object boxes, learning to reverse the diffusion from ground truth during training and iteratively refining randomly generated boxes during inference, offering flexibility in the number of boxes and evaluation method. StyleSwin\cite{zhang2022styleswin} is a high-resolution image synthesis framework using a pure transformer-based generative adversarial network, incorporating Swin transformer in a style-based architecture with double attention for larger receptive fields and absolute position knowledge, enhanced by a wavelet discriminator to overcome blocking artifacts and maintain spatial coherence.Yang \textit{et al.} \cite{yang2023paint} advances exemplar-guided image editing by employing self-supervised training to skillfully disentangle and rearrange elements from a source image and an exemplar, using an information bottleneck and strong augmentations to avoid copy-paste artifacts, and introducing an arbitrary shape mask with classifier-free guidance for enhanced control, all within a single forward pass of a diffusion model. Whang \textit{et al.} \cite{whang2022deblurring} utilizes conditional diffusion models to train a stochastic sampler that refines outputs from a deterministic predictor, offering a diverse set of perceptually superior reconstructions for a given blurred input, while also achieving efficiency in sampling and competitiveness in standard distortion metrics like PSNR.

